Speakers Unembedded: Embedding-free Approach to Long-form Neural Diarization

End-to-end neural diarization (EEND) models offer significant improvements over traditional embedding-based Speaker Diarization (SD) approaches but falls short on generalizing to long-form audio with large number of speakers. EEND-vector-clustering method mitigates this by combining local EEND with global clustering of speaker embeddings from local windows, but this requires an additional speaker embedding framework alongside the EEND module. In this paper, we propose a novel framework applying EEND both locally and globally for long-form audio without separate speaker embeddings. This approach achieves significant relative DER reduction of 13% and 10% over the conventional 1-pass EEND on Callhome American English and RT03-CTS datasets respectively and marginal improvements over EEND-vector-clustering without the need for additional speaker embeddings. Furthermore, we discuss the computational complexity of our proposed framework and explore strategies for reducing processing times.

==> abstract_xiang.tex <==
\begin{abstract}

Recently, a hybrid speaker diarization system was proposed to combine the advantages of both clustering-based and end-to-end neural diarization (EEND)-based frameworks, becoming the state-of-the-art. This system is performed in a local-global fashion: an EEND model is used for local speaker labeling and embeddings are computed for speakers seen in each local window; a global clustering is further applied to tie the same speaker across the local windows. Instead of involving speaker embedding module with additional training effort, in this paper, we propose a novel and simple embedding-free approach by applying EEND only, for both local and global steps. Inter-window label permutation after local EEND is solved by applying EEND again on pairwise input features between every two speakers across local windows to get speaker-pairwise scores where clustering is further performed to obtain global speaker ids. Experimental results on NIST CALLHOME show this approach can outperform its counterpart EEND-vector-clustering approach with both oracle and estimated number of speakers. Significant DER reduction over conventional 1-pass EEND is observed on other benchmarks with longer recordings. The issue of computation complexity in the global step is discussed, which reveals the potential for further improvement.

\end{abstract}

==> conclusion_xiang.tex <==
\section{Conclusion}

In this paper, we propose a novel embedding-free diarization approach which only applies EEND on both local and global steps. The global clustering is achieved without the usage of speaker embeddings by applying EEND to recreated pair-wised speaker features between every two speakers across local windows to get speaker-pairwise scores where clustering is further performed to obtain global diarization. This approach outperforms its counterpart EEND-vector-clustering approach on NIST CALLHOME and beats the conventional 1-pass approach on other widely used diarization benchmarks. We also discussed the computation complexity in the global EEND step and propose the potential further improvements.


==> experiments_xiang.tex <==
\section{Experiments}

In this section, we described the data construction, EEND model and clustering settings for reproduction. Improvements during adaptation and efficient inference are also introduced.

\subsection{Data and metrics}

Data is prepared for training, adaptation and evaluation, respectively. For the training, we generate simulated mixtures by mixing Switchboard-2 (Phase I \& II \& III), Switchboard Cellular (Part 1 \& 2), and the NIST Speaker Recognition Evaluation (2004 \& 2005 \& 2006 \& 2008) with MUSAN corpus \cite{snyder2015musan}, following the data generation procedure in \cite{fujita2019end}. Mixtures with up to 3 speakers were created, with $\beta=[2, 2, 9]$ for mixture with 1, 2 and 3 speakers, respectively. 

For adaptation and evaluation, real telephone conversation dataset CALLHOME \cite{przybocki2000martin}, i.e., NIST SRE2000 (LDC2001S97, Disk-8) is used. It is widely used as the benchmark for existing EEND-based approaches. The CALLHOME dataset contains 500 sessions, each with 2 to 6 speakers. There are two dominant speakers in each conversation. We split it into two subsets according to \cite{horiguchi2020end} for adaptation and evaluation, respectively. 

As local-global based framework is designed for dealing with long conversations, to show the effectiveness of this framework, evaluations on other benchmarks with longer audios are reported as well, such as CALLHOME American English (CHAE) \cite{canavan1997nist} and RT03-CTS \cite{fiscus2007nist}. We used the official splits for test sets.

For evaluation metrics, we use the diarization error rate (DER) \cite{nist2009evaluation} with a collar tolerance of 250ms. Overlapping speech segments are included in the evaluation.

\subsection{EEND model settings}

To guarantee a fair comparison with the existing hybrid baseline, we follow the front-end setting in the EEND-vector-clustering where 23-dimensional log-Mel-filterbank features are extracted, with a frame length of 25ms and frame shift of 10ms. The window size $T$ is set as 300 (=30s) for both training and adaptation. As EEND architecture, we use 6 stacked self-attention-based Transformer layers with eight attention heads and 256 hidden size, aligning with the setting in the EEND-vector-clustering as well.  In each window, the EEND model estimates the posteriors of 3 speakers.

The Adam optimizer \cite{kingma2014adam} is used during training and adaptation, with the Noam scheduler \cite{vaswani2017attention} and 150,000 warm-up steps for training and a fixed learning rate of $1\times$$10^{-5}$ for adaptation. Both are trained for 100 epoches.

\subsection{Sequence concatenation during adaptation}

In global EEND step, we create the chunk-level input by concatenating frame-level acoustic features between every two speakers across local windows, resulting in a new speaker-pairwise sequence which has not been seen before in both training and adaptation data. To get EEND generalized better to this input format, we include such data generation procedure during adaptation. Specifically, for each batch, half of the adaptation data are reformatted by first aggregating the frame-level acoustic features coming from the same speaker in each utterance to several blocks and concatenating every two blocks to generate a new input utterance. Overlapping frames are filtered out at the beginning.

% \subsection{Clustering setting}

% We performed the clustering using two algorithms, AHC and SC, by introducing constraint into different speakers detected in each local window in the local-EEND step. 
% %Other algorithms may not be suitable as we can only apply pre-computed distance matrix/similarity matrix instead of embeddings.
% Cannot-link speaker pairs are obtained from the detected different speakers in each local window in the local EEND step, such as $speaker 1$ and $speaker 2$ in the Figure 1. For constraint AHC, the distance for cannot-link speakers is set as $1e+4$. For constraint SC, the similarity for cannot-link speakers is set as 0. 

\subsection{Efficiency improvement for inference}

In the global step, during inference, each speaker in a window is paired with each speaker in subsequent windows. Hence the computational complexity will be $O(n^2)$. As shown in Figure 1, if there are 3 windows with each window containing 2 speakers, there will be 12 inference calls in global EEND step. RealTimeFactor(RTF) is used as a criteria to measure the efficiency of SD systems. RTF is calculated by dividing the time taken by the SD system by the total duration of the spoken audio. 
Normally, global EEND step during inference is performed in a sequential way which means for the given example in Figure 1, 12 inference calls were made one after the other which wont result in full utilization of GPU. In order to improve GPU utilization and reduce RTF, multiple inference requests can be batched together. We also attempt to reduce the number of frames of each speaker during global-EEND inference, which will further reduce the amount of computations during inference. Three different strategies were attempted. 1) taking first-N frames (N=50,100,150,200) of each speaker; 2) sub-sampling frames of each speaker by a factor of 2; 3) randomly selecting N frames of each speaker where N can be maximum 30,50 and 100 frames. 

% \begin{equation} \tag{3}
% \boldsymbol{I_1,..., I_{S_{Global}}} = AHC(\textbf{D})
% \end{equation}

% \begin{equation} \tag{4}
% \boldsymbol{I_1,..., I_{S_{Global}}} = SC(\textbf{S})
% \end{equation}


==> introduction_xiang.tex <==
\section{Introduction}

Speaker diarization (SD) is the process of partitioning an audio stream with multiple speakers into homogeneous segments associated with each speaker. It is often referred to as “who spoken when” problem. A conventional diarization system is typically consist of separate modules \cite{anguera2012speaker, sell2014speaker, snyder2016deep, garcia2017speaker, sell2018diarization, wang2018speaker}: voice activity detection, embedding extraction and clustering. This family of approaches shows advantages in dealing with long-form audio containing an arbitrary number of speakers. However, it has difficulties in handling overlapping speech and several separate modules may also lead error propagation. 

To overcome these drawbacks, end-to-end neural diarization (EEND) is proposed, formulating SD as a simple frame-wise multi-label classification problem with permutation invariant training \cite{fujita2019end}. It allows multiple speakers to be active simultaneously, thus it can handle overlapping speech naturally. Despite EEND and its further variants (e.g., EEND-SA \cite{fujita2019endsa}, EEDN-EDA \cite{horiguchi2020end}, etc) in theory showing much promise, generalization to arbitrarily long conversations ($>$ few minutes) and for larger number of speakers ($>$4) have been challenging. A few recent works took a step back and proposed a hybrid framework such as EEND-vector-clustering \cite{kinoshita2021integrating, kinoshita2021advances}, which integrates EEND and the conventional multi-module (i.e., clustering-based) approach. It typically works in a local-global fashion: leveraging the power of EEND for local speaker labelling in short windows (15-30 seconds) while computing embeddings for speakers seen in each local window; A global clustering is further performed on speaker embeddings to tie the same speaker across windows. This hybrid framework can deal with both overlapping speech due to local EEND and long conversations with arbitrary number of speakers due to global clustering, which makes the best of both worlds.

Most of the improvements on EEND framework are focused on the integration of additional embedding \cite{kinoshita2021integrating, kinoshita2021advances, zeghidour2021dive, yu2022auxiliary, fung2023robust, wang2023end} or attractor \cite{horiguchi2021towards, rybicka2022end, fujita2023neural, hao2023end, chen2023attention, samarakoon2023transformer} modules, which may require effort on specific model architecture and loss function design. Instead of involving additional speaker embeddings, in this paper, we propose a novel embedding-free approach built on top of the hybrid local-global framework. Its most striking advantage is it only applies common-used vanilla EEND model, both locally and globally, thus called local-global EEND. It consists of three steps: local EEND, global EEND and clustering. 
% Global clustering without the usage of speaker embeddings is achieved by applying EEND to speaker-pairwise inputs between local windows to get pair-wised scores. 
In local EEND step, the long input audio is first split into smaller chunks with a fixed window size (e.g., 15-30s). Then an EEND is applied to each local window for the diarization results, which is the same as the local step in EEND-vector-clustering but without further embedding extraction. 
The global EEND step innovatively solves the inter-chunk label permutation problem by performing chunk-level EEND again, to recreated speaker-pairwise chunks. Specifically, frame-level acoustic features of every two speakers across local chunks are paired, to form new chunks. The same EEND is applied to generate frame-level speaker posteriors where speaker-pairwise scores can be further computed. Such process is repeated between every two speakers across windows, in order to form an affinity/distance matrix where clustering is finally performed to obtain global speaker ids, thus achieving embedding-free speaker diarization.

In the rest of the paper, we first introduce the proposed local-global EEND in section 2, especially how the global step is performed. Then, the experimental settings are described in section 3. In section 4, we demonstrate the experimental results on several benchmarks, such as NIST CALLHOME, CALLHOME American English and RTCTS, compared with 1-pass conventional EEND and other local-global baselines. We will also discuss the computation complexity in global step which can be potentially improved.

==> local_global_xiang.tex <==
\section{Local-global EEND}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{local-global-EEND-v3.png}
  \caption{Local-global EEND diagram.}
  \label{fig:local_global_eend}
\end{figure*}

\subsection{Local EEND}
Figure 1 shows the schematic diagram of the proposed embedding-free approach which can be divided into local EEND, global EEND and clustering steps.

The local step is actually the same as that in EEND-vector-clustering. The input audio is first split into $N$ chunks with a fixed window length. We set $N$ as 3 in Figure 1 for the sake of simplicity. In each chunk $i$, frame-level acoustic features are extracted, denoted as $\textbf{X}_i = \{\textbf{x}_{i,t}\}_{t=1}^{T}$ where $t$ and $T$ are the frame index and window/chunk size, respectively. $\textbf{x}_{i,t}\in\Bbb{R}^F$ is an $F$-dimensional Mel-filterbank feature. Speaker label $\textbf{y}_{i,t}=\{y_{i,t,c} \in \{0,1\}\}_{c=1}^{C}$ denotes a joint activity for $C$ speakers at frame $t$. an EEND model estimates frame-wise posteriors $P(y_{i,t,c}|{\textbf{X}_i})$ in each window using a neural network.

As the EEND is applied to each local window independently, only local diarization results within each window can be obtained while label permutation issue across windows is remained.  In EEND-vector-clustering, this permutation issue is solved by extracting speaker embeddings for speakers seen in each local window, and then a clustering is applied on embeddings to obtain global diarization results. An additional joint optimized embedding module alongside EEND is used.

Instead of using speaker embeddings to achieve global clustering, an embedding-free global step is proposed in this paper. In global EEND step, we recreate each chunk by pairing the frame-level acoustic features between every two speakers across local windows, and EEND is again applied to get speaker-pairwise scores where an affinity/distance matrix can be formed. Finally, the global clustering is performed on this pre-computed affinity/distance matrix, thus achieving embedding-free approach.

\subsection{Global EEND}
According to the diarization results from local EEND step, the overlapping input frames are first filtered out, and remaining frames of the each speaker in each window will be paired with the ones of each speaker in subsequent windows, resulting in new speaker-pairwise chunks
\begin{equation} \tag{1}
\hat{\textbf{X}}_{i} = concat(\textbf{x}_{j,t} | t=[m_j, ..., m_T], \textbf{x}_{k,t} | t=[n_k, ..., n_T])
\end{equation}
 representing acoustics features from speaker $m$ corresponding to frame indexes $[m_j,..., m_T]$ in local window $j$ are concatenated with those from speaker $n$ corresponding to frame indexes $[n_k,..., n_T]$ in local window $k$, resulting in a new input sequence $\hat{\textbf{X}}_{i}$ in local window $i$ in the global step. The EEND is applied to $\hat{\textbf{X}}_{i}$ to generate frame-level speaker posteriors $\hat{P}(y_{i,t,c}|{\hat{\textbf{X}}_{i}})$
\begin{equation} \tag{2}
[\textbf{z}_1, ...,\textbf{z}_{T_m}, \textbf{z}_{T_m+1}, ..., \textbf{z}_{T_n} ] = EEND(\hat{\textbf{X}}_{i})
\end{equation}
where $\{\textbf{z}_t\}_{t=1}^{T_n}$ are the frame-wise posteriors where $\textbf{z}_t \in\Bbb{R}^C$. $[\textbf{z}_1, ...,\textbf{z}_{T_m}]$ and $[\textbf{z}_{T_m+1}, ..., \textbf{z}_{T_n}]$ correspond to the posteriors from speaker $m$ and $n$ respectively.
 This process is performed on every two speakers across local windows. 
 % The computation complexity should be proportional to the number of local windows and number of detected speakers in each window in local EEND step, which results in $N \times C$ in maximum. 
 As shown in Figure 1, we take the frames from $speaker 1$ and concatenate them with the frames from $speaker 3$ to create a new input sequence which is then fed into the EEND model. The same process is repeated between $speaker 1$ and $speaker 4$, $speaker 1$ and $speaker 5$, etc. 
 % This allows us to maintain speaker label fidelity across different local windows.

\subsection{Embedding-free clustering}

In the global EEND step, the output frame-wise posteriors $\{\textbf{z}_t\}_{t=1}^{T_n}$ are further averaged on frames belonging to the same speaker, resulting in speaker-level posteriors $\overline{\textbf{z}}_m$ and $\overline{\textbf{z}}_n$. Speaker-pairwise score $S_{mn}$ is further measured between them.
\begin{equation} \tag{3}
\overline{\textbf{z}}_m = average([\textbf{z}_1, ...,\textbf{z}_{T_m}])
\end{equation}
\begin{equation} \tag{4}
\overline{\textbf{z}}_n = average([\textbf{z}_{T_m+1}, ..., \textbf{z}_{T_n}])
\end{equation}
\begin{equation} \tag{5}
S_{mn} = cosine\_simalirity(\overline{\textbf{z}}_m, \overline{\textbf{z}}_n)
\end{equation}
Each $S_{mn}$ is an entry of the affinity matrix $\textbf{S}\in\Bbb{R}^{S_{Global}\times S_{Global}}$ which is used for final clustering. $S_{Global}$ is the number of total different speakers detected in every local window in local EEND step, such as $S_{Global}=6$ in Figure 1.

A cannot-link constraint can be used in the clustering algorithms between existing different speakers detected in each local window from the local EEND step, to prevent this pair from being assigned to the same speaker cluster. Spectral Clustering (SC) is chosen regarding our preliminary experiments. Constraint is introduced by setting a value of 0 (e.g., $D_{12}=0$) to cannot-link speaker pairs.
\begin{equation} \tag{6}
\boldsymbol{I_1,..., I_M} = \textit{SpectralClustering}(\textbf{S})
\end{equation}
SC performs a series of transformations on the affinity matrix to produce an eigen space $\{\boldsymbol{v_i}\}_{i=1}^{S_{Global}}$ where $\boldsymbol{v_i} \in \mathbb{R}^{1\times M}$ and $M$ is the number of speaker clusters detected by the maximum eigen-gap of the eigen values. K-Means is applied to these eigen space embeddings to group $S_{Global}$ speakers into cluster sets \(\{\boldsymbol{I_j}\}_{j=1}^M\).

\begin{table*}
  \caption{Effect of sequence concatenation on CALLHOME2.}
  \label{tab:seq_concate}
  
  \centering
  % \addtolength{\tabcolsep}{-3pt}
  % \scalebox{0.7}{%
  \begin{tabular}{ccccccc|c}
    \toprule
    \multirow{2}*{System} & \multirow{2}*{Model} & \multicolumn{6}{c}{\# of speakers in a session} \\
    & & 2 & 3 & 4 & 5 & 6 & all \\
    \midrule
    \multirow{2}*{1-pass EEND} & $Model_{local}$ & 7.53 & 14.91 & - & - & - & - \\
    & $Model_{local\_concat}$ & 7.36 & 17.74 & - & - & - & - \\
    \midrule
    \multirow{3}*{local-gloabl EEND} & $Model_{local}$ & 7.99 & 12.21 & 16.39 & 17.10 & 26.12 & 12.48 \\
    % 10.58\\
    & $Model_{local\_concat}$ & \textbf{7.29} & 11.85 & 17.83 & \textbf{15.76} & \textbf{22.38} & \textbf{12.16} \\
    % & 10.16\\
    & $Model_{local}+Model_{local\_concat}$ & 7.66 & \textbf{11.67} & \textbf{16.03} & 17.56 & 23.71 & 12.45 \\
    % & 10.43\\
    
    \bottomrule
  \end{tabular}
  
\end{table*}


==> results_xiang.tex <==
\section{Results}

We first evaluated the effect of sequence concatenation in the adaptation, and further compared the proposed approach with existing baselines by using oracle and estimated number of speakers during clustering. We also report the results on other widely used benchmarks, like CALLHOME American English (CHAE) and RTCTS. Finally, we do analysis on the improvement of efficiency in the global EEND inference.

\subsection{Effect of sequence concatenation}

We tried two kinds of input data format during adaptation, resulting in $Model_{local}$ and $Model_{local_concate}$ where the former denotes the model adapted with original input sequences that are normally used during EEND model adaptation while the latter is the one adapted with a combination of original sequences and concatenated sequences as described in section 2.2. We compare the proposed local-global EEND with the 1-pass conventional EEND, using different adaptation models in Table 1. The oracle speaker information is used during global clustering. We pick the best DER score for 1-pass EEND by looping the binarization thresholds from 0.3 to 0.7. Local-global EEND outperforms 1-pass EEND on $Model_{local}$ by 18\% on 3-speaker session while degrades the performance on 2-speaker session. Then $Model_{local\_concate}$ makes up the gap, which further improves the performance over $Model_{local}$ for local-global EEND by 8.8\% and 3\% on 2-speaker and 3-speaker sessions, respectively. For 1-pass EEND, $Model_{local\_concate}$ only benefits for the 2-speaker session but not for the 3-speaker one, which is expected due to the data mismatch between adaptation and evaluation where concatenation during adaptation only happens on pairwise speakers. When more number of speakers are evaluated for local-global EEND, $Model_{local\_concate}$ consistently performs better, except from 4-speaker session. Due to different input statistcs between local and global EEND steps, we also attempt to apply $Model_{local}$ in local EEND while $Model_{local\_concate}$ in global EEND, which further improves the performance on 3- and 4-speaker sessions. Generally, applying $Model_{local\_concate}$ only in both steps can achieve the desirable results regarding the DER on all speakers.

\begin{table}
  \caption{Comparison with other baselines with oracle number of speakers.}
  \label{tab:seq_concate}
  \centering
  \addtolength{\tabcolsep}{-3pt}
  \scalebox{0.8}{%
  \begin{tabular}{cccccc|c}
    \toprule
    \multirow{2}*{System} & \multicolumn{5}{c}{\# of speakers in a session} \\
    \cline{2-6} & \\[-1.0em]
    & 2 & 3 & 4 & 5 & 6 & all \\
    \midrule
    x-vector-clustering \cite{horiguchi2020end} & 8.93 & 19.01 & 24.48 & 32.14 & 34.95 & 18.98 \\
    EDA-EEND \cite{horiguchi2020end} & 8.35 & 13.20 & 21.71 & 33.00 & 41.07 & 15.43 \\
    EEND-vector-clust. (T=30s) \cite{kinoshita2021advances} & 8.08 & \textbf{11.27} & \textbf{15.01} & 23.14 & 26.56 & 12.22 \\
    
    \midrule
    % 1-pass EEND &  \\
    % \midrule
    local-gloabl EEND & \textbf{7.29} & 11.85 & 17.83 & \textbf{15.76} & \textbf{22.38} & \textbf{12.16}\\
    % local-gloabl EEND ($Model_{local}+Model_{local\_concat}$) & 7.66 & 11.67 & 16.03 & 17.56 & 23.71 & 12.45\\
    
    \bottomrule
  \end{tabular}}
  
\end{table}

\begin{table}[t]
  \caption{Comparison with other baselines with estimated number of speakers.}
  \label{tab:seq_concate}
  \centering
  \addtolength{\tabcolsep}{-3pt}
  \scalebox{0.8}{%
  \begin{tabular}{ccccccc}
    \toprule
    \multirow{2}*{System} & \multicolumn{5}{c}{\# of speakers in a session} \\
    \cline{2-6}& \\[-1.0em]
    & 2 & 3 & 4 & 5 & 6 & all \\
    \midrule
    x-vector-clustering & 15.54 & 18.01 & 22.68 & 31.40 & 34.27 & 19.43 \\
    EDA-EEND & 8.50 & 13.24 & 21.46 & 33.16 & 40.29 & 15.29 \\
    EEND-vector-clust. (T=30s) \cite{kinoshita2021advances} & 7.96 & 11.93 & 16.38 & 21.21 & 23.10 & 12.49 \\
    EEND-EDA-local-global \cite{horiguchi2021towards} & \underline{7.11} & \underline{11.88} & \underline{14.37} & 25.95 & \underline{21.95} & \underline{11.84} \\
    \midrule
    % 1-pass EEND &  \\
    % \midrule
    local-gloabl EEND & \textbf{7.51} & 12.20 & 17.88 & \textbf{16.01} & \textbf{22.35} & 12.20 \\
    % local-gloabl EEND ($Model_{local}+Model_{local\_concat}$) & 7.70 & 11.97 & 16.41 & 18.64 & 23.43 & 12.53\\
    
    \bottomrule
  \end{tabular}}
  
\end{table}



\subsection{Comparison with other baselines}

Table 2 and Table 3 show the performance of 
local-global EEND, compared with other baselines, with oracle and estimated number of speakers, respectively. We pick the results for EEND-vector-clustering with a window size of 30s from their paper and report the results for local-global EEND with $Model_{local_concate}$ only for both local and global EENDs. For oracle number of speakers, except from 3- and 4-speaker sessions, local-global EEND outperforms the EEND-vector-clustering on the other sessions where 5- and 6-speaker sessions show the significant improvement by 32\% and 15.7\%, respectively. The degradation on 4-speaker session may result from the undesirable window size, which is observed in the EEND-vector-clustering paper as well, indicating different window size may lead to large variation on the performance with more number of speakers. 

In table 3 for the results with estimated number of speakers, we include another latest baseline EEND-EDA-local-global with 6 blocks which is aligned with the number of blocks in EEND-vector-clustering and our local-global EEND. Compared with EEND-vector-clustering, we achieve better performance on all-speaker seesion and on almost all the sessions, still except from 3- and 4-speaker ones. Compared with EEND-EDA-local-global, we show slightly worse performance on $\{2, 3, 6\}$- speaker sessions but significantly better performance on 5-speaker session. The difference can potentially come from different amount of training data. Local-global EEND is
trained with up to 3-speaker mixtures while EEND-EDA-local-global is trained with up to 4-speaker mixtures which contains 100,000 more 4-speaker training mixtures. Therefore, it achieves the best score on 4-speaker session as expected.

\begin{table}
  \caption{DER (\%) on other benchmarks ($Th_{local}$=0.5).}
  \label{tab:seq_concate}
  \centering
  % \addtolength{\tabcolsep}{-3pt}
  \scalebox{0.9}{%
  \begin{tabular}{cccc}
    \toprule
    \multirow{2}*{System} & \multicolumn{3}{c}{Dataset}  \\
    \cline{2-4} & \\[-2.0ex]
    & CHAE test & CHAE 109 & RTCTS test\\
    \midrule
    1-pass EEND & 5.95 & 7.25 & 5.69\\
    local-global EEND & 5.20 & 7.02 & 5.14\\
  
    \bottomrule
  \end{tabular}}
  
\end{table}

\subsection{Performance on other benchmarks}

Other widely used diarization benchmarks, like CALLHOME American English (CHAE) and RTCTS are adopted to further evaluate the performance of local-global EEND. These datasets are consist of audios with longer duration, which can reveal the effectiveness of local-global systems. A fixed threshold (=0.5) is used for binarization to get diarization results and local-global EEND is based on estimated number of speakers. As shown in Table 4, local-global EEND can beat 1-pass EEND by 12.7\%, 3\% and 9.7\% on CHAE test, CHAE 109 and RTCTS test sets, respectively.


\subsection{Inference Efficiency improvement results}
Figure-2 shows results of different inference experiments on CALLHOME American English. All the experiments are performed on NVIDIA A10 GPU on AWS cloud(G5-2xLarge). Based on experiments, it is found that moving from sequential inference to batching (batching 500 pairs) reduced RTF by 50\%. Further RTF reduction were gained by reducing computation by selection subset of frames in global EEND either by selecting first N frames or random N frames. Figure-2 shows results with random N frames because random-N frames achieves RTF gains without impacting WER till N=50. Hence best results are with random N=50 frames.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{RTF_vs_DER.png}
  \caption{RTF vs DER with different inference experiments. It shows random 50 samples in global EEDN produces best result.}
  \label{fig:RTF_vs_DER}
\end{figure}



% \section{Discussion}

% Discuss about computation complexity in the global EEND step and propose further improvements.

